Joint Transmit Signal and Beamforming Design for Integrated Sensing and Power Transfer Systems

Integrating different functionalities, conventionally implemented as dedicated systems, into a single platform allows utilising the available resources more efficiently. We consider an integrated sensing and power transfer (ISAPT) system and propose the joint optimisation of the rectangular pulse-shaped transmit signal and the beamforming vector to combine sensing and wireless power transfer (WPT) functionalities efficiently. In contrast to prior works, we adopt an accurate non-linear circuit-based energy harvesting (EH) model. We formulate and solve a non-convex optimisation problem for a general number of EH receivers to maximise a weighted sum of the average harvested powers at the EH receivers while ensuring the received echo signal reflected by a sensing target (ST) has sufficient power for estimating the range to the ST with a prescribed accuracy within the considered coverage region. The average harvested power is shown to monotonically increase with the pulse duration when the average transmit power budget is sufficiently large. We discuss the trade-off between sensing performance and power transfer for the considered ISAPT system. The proposed approach significantly outperforms a heuristic baseline scheme based on a linear EH model, which linearly combines energy beamforming with the beamsteering vector in the direction to the ST as its transmit strategy.

==> Figures/optimal_tau.tex <==
\definecolor{black}{RGB}{0,0,0}
\definecolor{bluish-green}{RGB}{0,158,115}
\definecolor{darkgray176}{RGB}{176,176,176}

\begin{tikzpicture}
\begin{axis}[
scale only axis,
%axis y line*=left,
tick align=outside,
tick pos=left,
unbounded coords=jump,
xlabel={$\tau \,\text{[s]} \rightarrow$},
xmin=-0.25e-09, xmax=2.09899051726205e-08,
xtick style={color=black},
xtick={-2.5e-09,0,2.5e-09,5e-09,7.5e-09,1e-08,1.25e-08,1.5e-08,1.75e-08,2e-08,2.25e-08},
xticklabels={-0.25,0.00,0.25,0.50,0.75,1.00,1.25,1.50,1.75,2.00,2.25},
ylabel={$\phi(A^*_\tau, \boldsymbol{w}^*_\tau) \,\text{[µW]} \rightarrow$},
x tick scale label style={yshift=4pt},
y grid style={darkgray176},
ymin=-0.163332736429258, ymax=1.90548121836406,
ytick style={color=black},
grid=both,
grid style={line width=.1pt, draw=gray!10},
major grid style={line width=.2pt,draw=gray!50},
minor tick num=5,
legend cell align=left,
legend pos=north west,
legend style={
    at={(0,1)},
    legend columns=1,
    legend entries={S-C $P_\mathrm{avg}=0.5$ W, S-D $P_\mathrm{avg}=0.5$ W, S-D $P_\mathrm{avg}=0.1$ W, S-D $P_\mathrm{avg}=0.04$ W, S-D $P_\mathrm{avg}=0.033$ W}
    }
]
\addlegendimage{mark=x,black};
\addlegendimage{mark=x,orange};
\addlegendimage{mark=square,orange};
\addlegendimage{mark=o,orange};
\addlegendimage{mark=*,orange};

\addplot [mark=x,
semithick,
black]
table{%
x  y
2.01896547589305e-10 0.0117428601655119
5.96521560433171e-10 0.0635837718294386
1.00076069459081e-09 0.110448736874629
1.40499982874846e-09 0.155524957668358
1.8092389629061e-09 0.199374171176067
2.21347809706374e-09 0.242162411267479
2.61771723122138e-09 0.286441454333229
3.02195636537902e-09 0.330370512629064
3.42619549953667e-09 0.375454300200567
3.83043463369431e-09 0.418213181823784
4.23467376785195e-09 0.461114438025819
4.63891290200959e-09 0.503683798908818
5.04315203616724e-09 0.543694453861609
5.44739117032488e-09 0.581787831298148
5.85163030448252e-09 0.621917300845379
6.25586943864016e-09 0.661794699346824
6.66010857279781e-09 0.70088361653403
7.06434770695545e-09 0.739918375407684
7.46858684111309e-09 0.778356872964518
7.87282597527073e-09 0.812780912219346
8.27706510942837e-09 0.851699301986632
8.68130424358602e-09 0.888493827830138
9.08554337774366e-09 0.926841887548893
9.4897825119013e-09 0.967693605315651
9.89402164605894e-09 1.00385274058578
1.02982607802166e-08 1.03319158770937
1.07024999143742e-08 1.07148520026754
1.11067390485319e-08 1.10340055696209
1.15109781826895e-08 1.13995843181549
1.19152173168472e-08 1.17467618428258
1.23194564510048e-08 1.20792398870773
1.27236955851624e-08 1.24748032285761
1.31279347193201e-08 1.28011922498246
1.35321738534777e-08 1.31341409377891
1.39364129876354e-08 1.34588812938463
1.4340652121793e-08 1.37782925306345
1.47448912559507e-08 1.40957565266712
1.51491303901083e-08 1.4412806075205
1.55533695242659e-08 1.47269286981761
1.59576086584236e-08 1.50390022671688
1.63618477925812e-08 1.53489524508531
1.67660869267389e-08 1.56512551709294
1.71703260608965e-08 1.5949789530292
1.75745651950541e-08 1.62586449533943
1.79788043292118e-08 1.65501030007555
1.83830434633694e-08 1.684070871773
1.87872825975271e-08 1.71311079547625
1.91915217316847e-08 1.74109254187545
1.95957608658424e-08 1.76875537399885
2e-08 1.79762535184151
};

\addplot [mark=x,
semithick,
orange]
table{%
x  y
3.23034476142888e-09 0.0105071536516417
3.4218959873389e-09 0.021306386203788
3.76727315426934e-09 0.0448060408941804
4.11265032119978e-09 0.0832099627726625
4.45802748813022e-09 0.137237678793915
4.80340465506066e-09 0.186978965271753
5.14878182199109e-09 0.221021674551353
5.49415898892153e-09 0.264950184789137
5.83953615585197e-09 0.307622948691813
6.18491332278241e-09 0.341127816565236
6.53029048971285e-09 0.38610824589359
6.87566765664329e-09 0.418796574859918
7.22104482357373e-09 0.459270178819947
7.56642199050417e-09 0.495578813414074
7.91179915743461e-09 0.530306869627641
8.25717632436505e-09 0.565797650791982
8.60255349129549e-09 0.598401754984038
8.94793065822593e-09 0.632579943007725
9.29330782515637e-09 0.667044330787658
9.63868499208681e-09 0.703159883643864
9.98406215901725e-09 0.735788890226786
1.03294393259477e-08 0.76161052395683
1.06748164928781e-08 0.798337465972266
1.10201936598086e-08 0.826895764768083
1.1365570826739e-08 0.86132962901291
1.17109479936694e-08 0.888434230985222
1.20563251605999e-08 0.918314590306854
1.24017023275303e-08 0.94810337232901
1.27470794944608e-08 0.977676891645003
1.30924566613912e-08 1.0096181623869
1.34378338283216e-08 1.04445240378354
1.37832109952521e-08 1.07422263401209
1.41285881621825e-08 1.10239664610628
1.4473965329113e-08 1.13107748309168
1.48193424960434e-08 1.1584189158918
1.51647196629738e-08 1.18766531529088
1.55100968299043e-08 1.21394796336731
1.58554739968347e-08 1.24156673149543
1.62008511637652e-08 1.26805658989257
1.65462283306956e-08 1.29596259239695
1.6891605497626e-08 1.31318970587085
1.72369826645565e-08 1.33966203040199
1.75823598314869e-08 1.36871695730504
1.79277369984174e-08 1.38313891437104
1.82731141653478e-08 1.41049546114328
1.86184913322782e-08 1.43728999934779
1.89638684992087e-08 1.4612856739683
1.93092456661391e-08 1.48546452504196
1.96546228330696e-08 1.50933151082863
2e-08 1.53367943387233
};

\addplot [mark=square,
semithick,
orange]
table{%
x  y
3.23034476142888e-09 0.00847382403572739
3.4218959873389e-09 0.0167360660274523
3.76727315426934e-09 0.0424521689604407
4.11265032119978e-09 0.0821768198013861
4.45802748813022e-09 0.124680424819472
4.80340465506066e-09 0.172472168477549
5.14878182199109e-09 0.218095640353673
5.49415898892153e-09 0.259286530020191
5.83953615585197e-09 0.296921140884466
6.18491332278241e-09 0.342844484785794
6.53029048971285e-09 0.37805328554004
6.87566765664329e-09 0.415442471424659
7.22104482357373e-09 0.448636145390114
7.56642199050417e-09 0.486181448818843
7.91179915743461e-09 0.518720375735979
8.25717632436505e-09 0.558342971774891
8.60255349129549e-09 0.602036810398875
8.94793065822593e-09 0.632297337596266
9.29330782515637e-09 0.662146242508752
9.63868499208681e-09 0.700477847535815
9.98406215901725e-09 0.734713300691905
1.03294393259477e-08 0.761067481538803
1.06748164928781e-08 0.792861639145793
1.10201936598086e-08 0.824013790881974
1.1365570826739e-08 0.865855449492912
1.17109479936694e-08 0.888434230985222
1.20563251605999e-08 0.918314590306854
1.24017023275303e-08 0.94810337232901
1.27470794944608e-08 0.977676891645003
1.30924566613912e-08 1.0096181623869
1.34378338283216e-08 1.04445240378354
1.37832109952521e-08 1.07422263401209
1.41285881621825e-08 1.10239664610628
1.4473965329113e-08 1.13107748309168
1.48193424960434e-08 1.1584189158918
1.51647196629738e-08 1.18766531529088
1.55100968299043e-08 1.21394796336731
1.58554739968347e-08 1.24156673149543
1.62008511637652e-08 1.26805658989257
1.65462283306956e-08 1.29596259239695
1.6891605497626e-08 1.31318970587085
1.72369826645565e-08 1.33966203040199
1.75823598314869e-08 1.36871695730504
1.79277369984174e-08 1.38313891437104
1.82731141653478e-08 1.41049546114328
1.86184913322782e-08 1.44131352552604
1.89638684992087e-08 1.4421517432034
1.93092456661391e-08 1.46936235682694
1.96546228330696e-08 1.48978145583886
2e-08 1.51552085566524
};

\addplot [mark=o,
semithick,
orange]
table{%
x  y
3.23034476142888e-09 0.0132524618234487
3.4218959873389e-09 0.0272228321209282
3.76727315426934e-09 0.0620065575780867
4.11265032119978e-09 0.101515042954634
4.45802748813022e-09 0.155677580097892
4.80340465506066e-09 0.192912508542075
5.14878182199109e-09 0.226363311170712
5.49415898892153e-09 0.263610692201244
5.83953615585197e-09 0.300296881806225
6.18491332278241e-09 0.335628222383692
6.53029048971285e-09 0.351176090768781
6.87566765664329e-09 0.363402793146883
7.22104482357373e-09 0.387983670931564
7.56642199050417e-09 0.397534255023245
7.91179915743461e-09 0.412832083147594
8.25717632436505e-09 0.425780861291036
8.60255349129549e-09 0.443660580394633
8.94793065822593e-09 0.448403272401476
9.29330782515637e-09 0.462849024712523
9.63868499208681e-09 0.477543987906552
9.98406215901725e-09 0.497620449053194
1.03294393259477e-08 0.50146703772644
1.06748164928781e-08 0.516372212388483
1.10201936598086e-08 0.530332217276953
1.1365570826739e-08 0.54510688496109
1.17109479936694e-08 0.557219544138157
1.20563251605999e-08 0.575447354389411
1.24017023275303e-08 0.588298584123894
1.27470794944608e-08 0.586491333700958
1.30924566613912e-08 0.603977101666182
1.34378338283216e-08 0.598082757065305
1.37832109952521e-08 0.627555799772271
1.41285881621825e-08 0.627597014975384
1.4473965329113e-08 0.625229460994008
1.48193424960434e-08 0.645769955454525
1.51647196629738e-08 0.666497634472355
1.55100968299043e-08 0.673690074376905
1.58554739968347e-08 0.663178480402109
1.62008511637652e-08 0.685450598907737
1.65462283306956e-08 0.688101191271299
1.6891605497626e-08 0.686908559017686
1.72369826645565e-08 0.685826385588742
1.75823598314869e-08 0.700912461035787
1.79277369984174e-08 0.716698785532812
1.82731141653478e-08 0.708022282381415
1.86184913322782e-08 0.720955485298734
1.89638684992087e-08 0.731062490794383
1.93092456661391e-08 0.770455864759547
1.96546228330696e-08 0.775595005903069
2e-08 0.769312839252235
};

\addplot [mark=*,
semithick,
orange]
table{%
x  y
3.23034476142888e-09 0.0132524618234487
3.4218959873389e-09 0.0272228321209282
3.76727315426934e-09 0.0620065575780867
4.11265032119978e-09 0.101515042954634
4.45802748813022e-09 0.155677580097892
4.80340465506066e-09 0.192912508542075
5.14878182199109e-09 0.204558688334095
5.49415898892153e-09 0.214457834838729
5.83953615585197e-09 0.227829071612145
6.18491332278241e-09 0.233747896550439
6.53029048971285e-09 0.251720813288257
6.87566765664329e-09 0.253421502065545
7.22104482357373e-09 0.259678017034384
7.56642199050417e-09 0.273583606267705
7.91179915743461e-09 0.293971580374087
8.25717632436505e-09 0.293073374655275
8.60255349129549e-09 0.306504083243844
8.94793065822593e-09 0.298431460039415
9.29330782515637e-09 0.310475111079255
9.63868499208681e-09 0.319501088526453
9.98406215901725e-09 0.314879631605119
1.03294393259477e-08 0.328216126103093
1.06748164928781e-08 0.335702828254058
1.10201936598086e-08 0.341205409314219
1.1365570826739e-08 0.339754462946472
1.17109479936694e-08 0.3524610883412
1.20563251605999e-08 0.363716332936935
1.24017023275303e-08 0.364591379275607
1.27470794944608e-08 0.360690892399166
1.30924566613912e-08 0.379620961720178
1.34378338283216e-08 0.39103013776134
1.37832109952521e-08 0.390624542753635
1.41285881621825e-08 0.402056641606184
1.4473965329113e-08 0.404655700126167
1.48193424960434e-08 0.408376012595457
1.51647196629738e-08 0.405171156817008
1.55100968299043e-08 0.418908193897647
1.58554739968347e-08 0.428582419706937
1.62008511637652e-08 0.43615014360831
1.65462283306956e-08 0.444632484121872
1.6891605497626e-08 0.44777941143817
1.72369826645565e-08 0.433644338051106
1.75823598314869e-08 0.436463001956289
1.79277369984174e-08 0.42767097481737
1.82731141653478e-08 0.421182677845297
1.86184913322782e-08 0.437795663118798
1.89638684992087e-08 0.443094958990745
1.93092456661391e-08 0.443204012240774
1.96546228330696e-08 0.446186875747417
2e-08 0.453167759808257
};



\end{axis}

\end{tikzpicture}


==> Figures/results.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\definecolor{bluish-green}{RGB}{0,158,115}
\definecolor{yellow}{RGB}{240, 228, 66}
\definecolor{purple}{RGB}{148,103,189}
\definecolor{brown}{RGB}{165,42,42}
\definecolor{pink}{RGB}{255, 192, 203}


\begin{axis}[
name=boundary,
scale only axis,
%axis y line*=left,
tick align=outside,
tick pos=left,
unbounded coords=jump,
x grid style={darkgray176},
xmin=1.8, xmax=6.1,
xtick style={color=black},
xlabel={$R_\mathrm{min} \,\text{[m]} \rightarrow$},
y grid style={darkgray176},
ymin=0, ymax=7.03976440673382,
ylabel={$\phi(A^{*}_{\tau^*}, \boldsymbol{w}^{*}_{\tau^*}) \,\text{[µW]} \rightarrow$},
ytick style={color=black},
grid=both,
grid style={line width=.1pt, draw=gray!10},
major grid style={line width=.2pt,draw=gray!50},
minor tick num=5%,
%legend cell align=left,
%legend pos=north west,
%legend style={
%    at={(0,1)},
%    legend columns=1,
    % legend entries={$\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    % $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    % $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    % $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    % $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    % $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    % $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    % $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\}
    % }
]

% \addlegendimage{mark=x,black};
% \addlegendimage{mark=o,black};
% \addlegendimage{mark=x,orange};
% \addlegendimage{mark=o,orange};
% \addlegendimage{mark=x,blue};
% \addlegendimage{mark=o,blue};
% \addlegendimage{mark=x,bluish-green};
% \addlegendimage{mark=o,bluish-green};


\addplot [mark=x, semithick, black]
table{%
x  y
2 1.0797270838562
2.44444444444444 1.3441937966136
2.88888888888889 1.54341598778148
3.33333333333333 1.7614187296905
3.77777777777778 1.95912022652652
4.22222222222222 2.15494463508147
4.66666666666667 2.30876510646729
5.11111111111111 2.50759428878663
5.55555555555556 2.62415025392142
6 2.80003719833079
};\label{plot1}

\addplot [mark=o, semithick, black, dash dot, mark options={solid}]
table{%
x  y
2 0.117395794695598
2.44444444444444 0.144330171257791
2.88888888888889 0.165830743910227
3.33333333333333 0.170110727678974
3.77777777777778 0.198898966856649
4.22222222222222 0.221488758466901
4.66666666666667 0.217970375718498
5.11111111111111 0.254471395483298
5.55555555555556 0.260316965174488
6 0.266982626237846
};\label{plot2}

\addplot [mark=x, semithick, orange]
table{%
x  y
2 2.70233827956404
2.44444444444444 3.22470204933476
2.88888888888889 3.6784422054826
3.33333333333333 4.16003102374154
3.77777777777778 4.51515088193331
4.22222222222222 4.9140977008084
4.66666666666667 5.33642838716538
5.11111111111111 5.72038981018239
5.55555555555556 6.01646329340004
6 6.32004201167397
};\label{plot3}

\addplot [mark=o, semithick, orange, dash dot, mark options={solid}]
table{%
x  y
2 0.344727484028178
2.44444444444444 0.434578738047915
2.88888888888889 0.458615057264742
3.33333333333333 0.507444652067703
3.77777777777778 0.583489741221977
4.22222222222222 0.629576938919978
4.66666666666667 0.683652846060688
5.11111111111111 0.736921627772977
5.55555555555556 0.75742566313716
6 0.763710284118398
};\label{plot4}

\addplot [mark=x, semithick, blue]
table{%
x  y
2 1.2874799133374
2.44444444444444 1.52018310138681
2.88888888888889 1.75959400127686
3.33333333333333 1.96987724151717
3.77777777777778 2.17876653563047
4.22222222222222 2.3355837617024
4.66666666666667 2.44421591471669
5.11111111111111 2.6071743080861
5.55555555555556 2.72321195583042
6 2.95013397135758
};\label{plot5}

\addplot [mark=o, semithick, blue, dash dot, mark options={solid}]
table{%
x  y
2 0.128393513671242
2.44444444444444 0.140583022328867
2.88888888888889 0.172567123216132
3.33333333333333 0.184303362733421
3.77777777777778 0.220015337748749
4.22222222222222 0.232605364963252
4.66666666666667 0.208869216867996
5.11111111111111 0.246795268989638
5.55555555555556 0.253088919622418
6 0.275970726878753
};\label{plot6}

\addplot [mark=x, semithick, bluish-green]
table{%
x  y
2 2.77512234127875
2.44444444444444 3.35233057673397
2.88888888888889 3.76913546159244
3.33333333333333 4.20323201617983
3.77777777777778 4.61845704871405
4.22222222222222 5.02669752144111
4.66666666666667 5.41768720304212
5.11111111111111 5.77455274107129
5.55555555555556 6.0870666985347
6 6.35747612538115
};\label{plot7}

\addplot [mark=o, semithick, bluish-green, dash dot, mark options={solid}]
table{%
x  y
2 0.363135409608469
2.44444444444444 0.41140234640511
2.88888888888889 0.455663223570817
3.33333333333333 0.507441132252514
3.77777777777778 0.60160309192234
4.22222222222222 0.637159434985406
4.66666666666667 0.700406730509645
5.11111111111111 0.723930677760232
5.55555555555556 0.773629808862499
6 0.807174141558874
};\label{plot8}


\end{axis}

\node[draw,fill=white,column sep={between borders}, row sep={0pt},below right=0em] at (boundary.north west) {\small
    \begin{tblr}{
        row{1} = {abovesep=-1pt,belowsep=-1pt},
        row{2} = {abovesep=-1pt,belowsep=-1pt},
        row{3} = {abovesep=-1pt,belowsep=-1pt},
        row{4} = {abovesep=-1pt,belowsep=-1pt},
        column{1} = {leftsep=-1pt,rightsep=1pt},
        column{2} = {leftsep=-1pt,rightsep=1pt},
        column{3} = {leftsep=1pt,rightsep=1pt},
        }
    \ref{plot1} & \ref{plot2} & $\hat{R}=0.05$ m, $P_\mathrm{p}=0.5$ W\\
    \ref{plot3} & \ref{plot4} & $\hat{R}=0.05$ m, $P_\mathrm{p}=1$ W\\
    \ref{plot5} & \ref{plot6} & $\hat{R}=1$ m, $P_\mathrm{p}=0.5$ W\\
    \ref{plot7} & \ref{plot8} & $\hat{R}=1$ m, $P_\mathrm{p}=1$ W\\
    \end{tblr}};

\end{tikzpicture}
